Simulating Parity Reasoning (extended version)

Propositional satisfiability (SAT) solvers, which typically operate using conjunctive normal form (CNF), have been successfully applied in many domains. However, in some application areas such as circuit verification, bounded model checking, and logical cryptanalysis, instances can have many parity (xor) constraints which may not be handled efficiently if translated to CNF. Thus, extensions to the CNF-driven search with various parity reasoning engines ranging from equivalence reasoning to incremental Gaussian elimination have been proposed. This paper studies how stronger parity reasoning techniques in the DPLL(XOR) framework can be simulated by simpler systems: resolution, unit propagation, and parity explanations. Such simulations are interesting, for example, for developing the next generation SAT solvers capable of handling parity constraints efficiently.

==> gesimulation.tex <==
\section{No polynomial Gaussian Elimination-simulation formulas}
\begin{lemma}
\label{Lem:GESimClause}
Given a satisfiable xor-clause conjunction $\phi$ in a conjunction $\xorclauses$
of xor-clauses such that $\xorclauses$ has a GE-simulation formula $\psi$ and the xor-clause conjunction $\xorclauses \wedge \psi$ is in 3-xor normal form, if $ \SetLC{\phi} \wedge \AL_1 \wedge \dots \wedge \AL_k \Models (\IL \equiv \parity{}) $ and $\SetLC{\phi} \not \Models (\IL \equiv \parity{}) $, then there is an xor-clause $ (z_1 \oplus z_2 \oplus \IL \equiv \parity{1} \oplus \parity{2} \oplus \parity{}) $ such that:
\begin{itemize}
\item $ \xorclauses \wedge \psi \Models (z_1 \equiv \parity{1}) \leftrightarrow (V_x' \oplus V_y \equiv \parity{1}') $
\item $ \xorclauses \wedge \psi \Models (z_2 \equiv \parity{2}) \leftrightarrow (V_x''\oplus V_y \equiv \parity{2}') $
\end{itemize}
\end{lemma}
where $V_x = \VarsOf{\SetLC{\phi}}$, $ (V_x',V_x'')$ is a partition of $V_x$, and $V_y \subset \LCVarsGone{\phi}$.

\begin{figure}
\centering
\begin{tabular}{p{0.9cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}p{0.75cm}}
$y_{1,4,7} \XX $ & $ x_1$ &           &           & $\XX$ & $ x_4$ &           &         & $\XX$  & $ x_7$ &           & & $\equiv \bot $ \\
$y_{2,5,8} \XX $ &           & $ x_2$ &           & $\XX$ &        & $ x_5$    &         & $\XX$  &           & $ x_8$ &  & $\equiv \bot $ \\
$y_{3,6,9} \XX $ &           &           & $ x_3$ & $\XX$ &        &           & $ x_6$  & $\XX$   &           &           & $ x_9$ & $\equiv \bot $  \\
$y_{1,5,9} \XX $ & $ x_1$ &           &           & $\XX$ &        & $ x_5$    &         & $\XX$  &          &          & $x_9$ & $\equiv \bot $ \\
$y_{2,6,7} \XX $ &           & $ x_2$ &           & $\XX$ &        &           & $ x_6$  & $\XX$  & $x_7$    &        &    & $\equiv \bot $ \\
$y_{3,4,8} \XX $ &           &           & $ x_3$ & $\XX$ & $x_4$  &           &        & $\XX$   &          &   $x_8$   &        & $\equiv \bot $  \\
\end{tabular}
\caption{A subset of xor-clauses in $G(1)$}
\label{Fig:SubsetG1}
\end{figure}

Let $G(1), \dots, G(n) $ be a family of xor-clause conjunctions over the variables $ \Set{x_1,\dots,x_{9n}} \cup \Setdef{y_{i,j,k}}{i,j,k \in \Set{1,\dots,n}}$ such that $G(n) = \bigwedge \Setdef{ (y_{i,j,k} \oplus x_i \oplus x_j \oplus x_k \equiv \bot) } {1 \leq i < j < k \leq 9n}$.
%\begin{itemize}
%\item if $1 \leq i < j < k \leq 9n$, then the xor-clause $ (y_{i,j,k} \oplus x_i \oplus x_j \oplus x_k \equiv \bot) $ is in $G(n)$
%\end{itemize}



\begin{theorem}
There is no GE-simulation formula $\psi$ for $G(n)$ such that $|\psi| = O(n^m)$ for some fixed $m$.
\end{theorem}

\begin{proof}
We first demonstrate that for the xor-clause conjunction $G(n)$ there are at least
$(9n)!$ sets of $6n$ variables such that by assigning $6n-1$ of the them, the
remaining one is the only xor-implied literal in the instance.
%
Let $ P(n) : \Set{1,\dots,9n} \rightarrow \Set{1,\dots,9n}$ be a permutation of
first $9n$ natural numbers.
%
Let $ Y_1(P) = \Setdef{y_{P(i),P(j),P(k)}}{1 \leq i \leq 3n, j = i+3n, k = i+6n}$ be a set of $3n$ variables 
and $ Y_2(P) = \Setdef{y_{P(i),P(j),P(k)}}{1 \leq i \leq 3n, j = 3n+1+(i+1 \mod 3n), k = 6n+1+(i+3n-1 \mod 3n)}$.
%
Let $ G_1(P) = \Setdef{C}{C \in G(n) \wedge \VarsOf{C} \subset Y_1(P)}$
and $ G_2(P) = \Setdef{C}{C \in G(n) \wedge \VarsOf{C} \subset Y_2(P)}$.
%
Figure~\ref{Fig:SubsetG1} has the xor-clauses $ G_1(P)$ and $G_2(P)$ where
$P(i) = i$.
%
Let $y' = y_{P(1),P(4),P(7)}$ and $ Y'(P) = (Y_1(P) \cup Y_2(p)) \setminus \set{y'}$.
%
There are $(9n)!$ permutations of the first $9n$ natural numbers, so it follows
that there are $(9n)!$ sets of $6n$ variables $Y'(P)$ such that $ G_1(P) \wedge
G_2(P) \bigwedge \Setdef{y \equiv \bot}{y \in Y'(P) } \Models
y_{P(1),P(4),P(7)}$, and thus $ G(n) \wedge \bigwedge \Setdef{y \equiv \bot}{y
\in Y'(P) } \Models (y' \equiv \bot)$.

Now assume that there is a GE-simulation formula $\psi$ for $G(n)$ such that
$|\psi| = O(n^m)$ for some fixed $m$. 
%
We can translate the xor-clause conjunction $ G(n) \wedge \psi $ to an equisatisfiable xor-clause conjunction $ G(n)' \wedge \psi' $ in 3-xor normal form such that $ |\psi'| = O(n^m)$.
%
It holds that $G(n)' \wedge  \psi' \wedge \Setdef{y \equiv \bot}{y
\in Y'(P) } \UPderiv (y' \equiv \bot)$.
%
By Lemma~\ref{Lem:LinearCombination}, there is a satisfiable xor-clause conjunction $\phi$ in $G(n)'$ such that $\SetLC{\phi} \wedge \Setdef{y \equiv \bot}{y \in Y'(P)} \Models (y' \equiv \bot) $ and $\SetLC{\phi} \not \Models (\IL \equiv \parity{})$.
%
By Lemma~\ref{Lem:GESimClause}, there is an xor-clause $ (z_1 \oplus z_2 \oplus \IL \equiv \parity{1} \oplus \parity{2} \oplus \parity{}) $ such that:
\begin{itemize}
\item $ G(n)' \wedge \psi' \Models (z_1 \equiv \parity{1}) \leftrightarrow (V_x' \oplus V_y \equiv \parity{1}') $
\item $ G(n)' \wedge \psi' \Models (z_2 \equiv \parity{2}) \leftrightarrow (V_x''\oplus V_y \equiv \parity{2}') $
\end{itemize}
where $V_x = \VarsOf{\SetLC{\phi}}$, $ (V_x',V_x'')$ is a partition of $V_x$, and $V_y \subset \LCVarsGone{\phi}$.
%
Note that for each permutation $P$, the corresponding set $V_x$ is different.
By the number of different permutations $P$ and above reasoning, there are
$(9n)!$ xor-clauses of the form $ (z_1 \oplus z_2 \oplus \IL \equiv
        \parity{1} \oplus \parity{2} \oplus \parity{}) $ in $G(n)' \wedge
\psi'$ which is a contradiction because we have assumed that $|\psi'| =
O(n^m)$. Thus, the theorem holds.
\end{proof}




